Constant Approximating Parameterized $k$-SetCover is W[2]-hard

In this paper, we prove that it is W[2]-hard to approximate k-SetCover within any constant ratio. Our proof is built upon the recently developed threshold graph composition technique. We propose a strong notion of threshold graphs and use a new composition method to prove this result. Our technique could also be applied to rule out polynomial time $o\left(\frac{\log n}{\log \log n}\right)$ ratio approximation algorithms for the non-parameterized k-SetCover problem with $k$ as small as $O\left(\frac{\log n}{\log \log n}\right)^3$, assuming W[1]$\neq$FPT. We highlight that our proof does not depend on the well-known PCP theorem, and only involves simple combinatorial objects.

==> derand.tex <==
\section{Derandomization}\label{sec:derand}
In this section, we show how to derandomized the reduction in Theorem~\ref{w1hardness}. It suffices to give a deterministic construct of an error correcting code $ C:\Sigma^r\to\Sigma^m$ with relative distance $\Delta( C)\ge 1-\frac{1}{(\log n)^{\Theta(1)}}$, $|\Sigma^r|=n^{\Theta(1)}$.  Note that the Reed-Solomon Code ${ C}^{RS}:\Sigma^r\to\Sigma^m$ has relative distance  $\Delta( C^{RS})= 1-\Theta(r/m)$ and $r\le m\le|\Sigma|$. To obtain a large relative distance   code while keeping  $|\Sigma|$ small,  we use the idea of concatenated codes.
%To obtain a large distance using Reed-Solomon Code, we have to set $\Sigma=\log n^{\Theta(1)}$ and $r=O(1)$, which violates the requirement  $|\Sigma^r|=n^{\Theta(1)}$.  To deal with this problem, we use the idea of concatenated codes.

\begin{definition}
Let $ C_{out} : \Sigma^r\to\Sigma^m$ and $ C_{in} : \Sigma'^R\to\Sigma'^M$ be two codes and $\Sigma'=\Sigma^r$, the concatenated code $C_{out}\circ C_{in} : \Sigma^{Rr}\to\Sigma^{Mm}$ is defined as follows.
For every $v_1,v_2,\ldots,v_R\in\Sigma'=\Sigma^r$, let $(u_1,\ldots,u_M)=C_{in}(v_1,\ldots,v_R)$. Define 
 $C_{out}\circ C_{in}(v_1,v_2,\ldots,v_R)=(C_{out}(u_1),\ldots,C_{out}(u_M))$.
\end{definition}
We have the following property for the concatenation of two codes~\cite{ECT}.
\begin{lemma}\label{lem:concat}
Let $\delta_1$ be the relative distance of $ C_{1}$ and $\delta_2$ be the relative distance of $ C_{2}$, then the relative distance of $ C_{1}\circ  C_{2}$ is $\delta_1\delta_2$.
\end{lemma}

\begin{theorem}[Derandomization of Theorem~\ref{w1hardness}]
Assuming  $\mathsf{W[1]} \neq \mathsf{FPT}$, there is no  polynomial time algorithm which can approximate non-parameterized {\sc $k$-SetCover} within $o\left(\frac{\log n}{\log\log n}\right)$ ratio, even if $k$ is as small as $O(\frac{\log^5 n}{\log\log n})$.
\end{theorem}
\begin{proof}
Similar to the proof of Theorem~\ref{w1hardness}, given an instance $(G,k)$ of $k$-Clique, let $\Gamma=(S,U,E)$ with $n=|S|$ and $|U|=k^3\log n$  be the instance of  \ksetcover{} obtained using Lemma~\ref{lem:setcoverw1}. Let $|\Sigma|=\log^2 n$, $|\Sigma'|=\log^4 n$, $r=2$, $R=\frac{\log n}{4\log\log n}$, $m=\log^2 n$, $M=\frac{\log^3 n}{8\log\log n}$. Let $\mathcal C_{1}:\Sigma^r\to\Sigma^m$ be the  Reed-Solomon Code with relative distance $1-r/m=1-2/\log^2n$. Let $\mathcal C_{2}:\Sigma'^R\to\Sigma'^M$ be the  Reed-Solomon Code with relative distance $1-R/M=1-2/\log^2n$.  By Lemma~\ref{lem:concat}, the distance of $C_{1}\circ C_{2}$ is $(1-2/\log^2n)^2\ge 1-4/\log^2n$. Applying Theorem~\ref{thm:reduction}, we construct a $(|\Sigma|^{rR},k,|\Sigma|^{k},mM,\frac{\log n}{2},1/2)$-threshold graph in time polynomial in $n$. Note that $|\Sigma|^{rR}=n$ and $mM=\frac{\log^5 n}{8\log\log n}$.
 Applying Theorem~\ref{thm:reduction} with $c\gets \frac{\log n}{k\log\log n}$,  $h\gets\frac{\log n}{2}$ and $m\gets mM=\frac{\log^5 n}{8\log\log n}$ and Lemma~\ref{lem:remove-weights}, we obtain an instance $\Gamma'$ of \setcover{} such that
 \begin{itemize}
     \item if $G$ contains a $k$-clique, then $\Gamma'$ has a solution of size $2mM$,
     \item if $G$ contains no $k$-clique, then the optimal solution has size larger than 
     \[
     \min\left\{mM \cdot\frac{\log n}{2k},mM\cdot\frac{\log n}{k\log\log n}\right\}=mM\cdot\frac{\log n}{k\log\log n}.
     \]
 \end{itemize}
%$(|\Sigma|^{rR},k,|\Sigma|^{k},\frac{\log^5n}{8\log\log n},\frac{\log n}{2},1/2)$
\end{proof}
%Recall that we require $|\Sigma|=(\log n)^{O(1)}$.

